A Survey on Sensor-based Threats to Internet-of-Things (IoT) Devices and Applications

The concept of Internet of Things (IoT) has become more popular in the modern era of technology than ever before. From small household devices to large industrial machines, the vision of IoT has made it possible to connect the devices with the physical world around them. This increasing popularity has also made the IoT devices and applications in the center of attention among attackers. Already, several types of malicious activities exist that attempt to compromise the security and privacy of the IoT devices. One interesting emerging threat vector is the attacks that abuse the use of sensors on IoT devices. IoT devices are vulnerable to sensor-based threats due to the lack of proper security measurements available to control use of sensors by apps. By exploiting the sensors (e.g., accelerometer, gyroscope, microphone, light sensor, etc.) on an IoT device, attackers can extract information from the device, transfer malware to a device, or trigger a malicious activity to compromise the device. In this survey, we explore various threats targeting IoT devices and discuss how their sensors can be abused for malicious purposes. Specifically, we present a detailed survey about existing sensor-based threats to IoT devices and countermeasures that are developed specifically to secure the sensors of IoT devices. Furthermore, we discuss security and privacy issues of IoT devices in the context of sensor-based threats and conclude with future research directions.

==> SideChannels.tex <==
\section{Side Channels of Various Cyber Physical Systems and IoT devices}
In this section, we give a detailed introduction of several side channels that are associated with IoT and CPS devices. Side channels are referred to non-conventional physical channels that can be used for establishing an unorthodox means of communication to exchange data from devices. Usually, in a device, data exchange is done via known communication channel like Bluetooth, Wi-Fi, etc. Side channels are different from these channels as they are more associated with application of the device rather than being used for communication purpose. Side channels carry various information like power consumption rate, electro-magnetic emission, acoustic behavior, sensor readings, etc. \par
General architecture of IoT and CPS devices has four layers. They are --- Perception layer, Network layer, Middle-ware or Processing layer, and Application layer \cite{farooq2015critical}. Detail description of these layers are given below.
\subsection{Perception Layer}
Main purpose of perception layer is to identify any phenomena in device peripheral and obtain data from the real world. Perception layer can also be described as sensing layer as it consists of several sensors. Primary purpose of using sensors in a device is to provide an interface between the device and physical phenomena occurred in the device ambiance. Using multiple sensors for applications is one of the primary features of IoT and CPS devices \cite{khan2012future}. Sensors in IoT devices can be categorized in three broad categories which are described below ---%When a task is being executed on a device, sensors in the perception layer can obtain some partial information about the data processed in network, middle-ware, and application layer. %As perception layer works as communication medium between device and ambience, such information can be revealed from the sensors, or can be obtained by an external device (power measurement tools, EM sensitive antenna, etc.). If there are \textit{N} possible ways of getting information from perception layer, we can assume that the device has \textit{N} number of side channels in it. An analogy can be given to understand the definition of side channel clearly. For example, keyboard is a common user input interface for various devices like laptop, cellphone, printer, etc. When a user types in keyboard, it generates several signals like acoustic signal, electro-magnetic signal, etc. These signals give a specific reading in corresponding sensors like microphone, gyroscope, etc \cite{1301311}. By performing certain analysis, we can infer the typed input correctly. For this scenario, microphone and gyroscope become side channels of the keyboard. \par

\subsubsection{Motion Sensor}
Motion sensors in IoT and CPS devices measure the change in motion of the devices as well as orientation of the devices. There are two types of motion change we can observe in a device. These are linear motion and angular motion. Linear motion refers to the linear displacement of a device while angular motion refers to the rotational displacement of a device. Different types of motion sensors are described in table~\label{sensors}.
\begin{enumerate}[(a)]
\item \textbf{Accelerometer:} Accelerometer is an electromechanical device which can measure changes in acceleration forces along lateral axis (x-axis), longitudinal axis (y-axis) and vertical axis (z-axis). Such measured acceleration forces can be a static force, like gravitational force, or a dynamic force caused by moving or vibrating. There are two working mechanisms used in accelerometer to measure acceleration forces. One mechanism uses piezoelectric effect in which accelerometers consist of a crystal structure that gets stressed by the change of acceleration force and generates a voltage. Another way to measure acceleration forces is to sense change in capacitance. If there are two structures next to each other, displacement in one structure will create a change in capacitance between them. This deviation in capacitance is then converted into voltage reading and acceleration forces can be calculated from this \cite{stanford}. In IoT and CPS devices with a graphical interface, accelerometer is used to detect various types of motion of the device like shake, tilt, etc. and adjust the orientation of the display accordingly. In smart vehicles, accelerometer is also used to measure the acceleration and velocity of the vehicles \cite{aram2012environment}.
\item \textbf{Linear acceleration sensor:} Linear acceleration sensor is used to monitor acceleration along a single axis. It is a type of accelerometer. The main difference between linear acceleration sensor and accelerometer is that accelerometer takes the effect of gravitational force into account while linear acceleration sensor only measures the change in motion. Linear acceleration sensor data can be computed from the data measured by accelerometer.
\item \textbf{Gyroscope:} Gyroscope measures the rate of change of angular momentum in all the three axis. Main feature of using gyroscope in IoT and CPS devices is to adjust orientation of the display according to angular momentum. Gyroscope can sense spin, turn, etc., which are used to detect human behavior by many apps \cite{wu2012classification}. 
\end{enumerate}

\begin{figure*}
  \includegraphics[width=\textwidth,height=12cm]{sensors}
  \caption{Sensors used in smart phones and smart watches}
\end{figure*}
\subsubsection{Environmental Sensor}
Various sensors have been embedded in IoT and CPS devices to sense the change in environmental parameters in device’s peripheral. Main purpose of using environmental sensor is to enable the devices to take autonomous decisions according to the changes of device peripheral. Environment sensors are also used in many applications to improve user experience e.g, home automation systems, smartphones, etc.. Some of the common environmental sensors used in IoT and CPS devices are ---
\begin{enumerate}[(a)]
\item \textbf{Light sensor:} Light sensor is common in every IoT and CPS device which has a display unit. Light sensors are typically photoresistors or photodiodes, which change characteristics with the change of light intensity. Two types of light sensors are used in IoT and CPS devices. They are --- ambient light sensor and RGBW sensor. Ambient light sensor only measures the intensity of the light while RGBW sensor can measure the light intensity of red, green, blue and white light and can distinguish between them. Main function of light sensor is to adjust the brightness and contrast of the display of a device according to the change of light intensity of the ambience.
\item \textbf{Proximity sensor:} Proximity sensor used in IoT and CPS devices is usually IR-based sensor which can detect the presence of nearby objects without any physical contact. As most of the IoT and CPS devices uses LCD display, proximity sensor is used to reduce display power consumption by turning off the LCD backlight. Proximity sensor is also used to disable the touch screen to avoid inadvertent touches while talking in smartphones \cite{web}.
\item \textbf{Temperature sensor:} Temperature sensor embedded in IoT and CPS devices measures temperature of the device as well as ambient temperature. Temperature sensor is vastly used in home automation appliances like \textit{Google NEST}, \textit{LG Smart AC}, etc.. 
\item \textbf{Acoustic sensor:} Acoustic sensor is used by the IoT devices for detecting audio and acoustic signals. Some CPS and IoT devices also use acoustic sensors for obstacle detection and navigation purpose \cite{rodriguez2012assisting}. There are two types of acoustic sensor used in IoT and CPS devices. Microphone, a common audio sensor, is used for many audio related applications like making phone calls and audio recording in smartphones and smart watches, taking audio input in voice command based apps in smartphones, navigation devices, etc.. Another acoustic sensor used in IoT and CPS devices is speaker. Speaker is usually used for playing audio files and listening audio feedbacks from applications. 
\item \textbf{Camera:} Modern CPS and IoT devices come with powerful camera which can take still pictures and record high definition video. Camera is considered as most impactful sensor because of the usability among common people \cite{camera}. The camera actually deals with several types of dataset which is related to device peripheral. For example, cameras in smartphones deal with light sensor and light intensity of the captured image can be adjusted. Again, video recording allows camera to interconnect with microphone and speaker of the device. So, camera can be considered not only as a sensor, but also as an interconnecting bridge of multiple sensors.
\end{enumerate}



\subsubsection{Position sensor}
Position sensor of IoT and CPS devices deals with physical position and location of the device. Most common position sensors used in IoT and CPS devices are magnetic sensor and GPS. These are described below ---
\begin{enumerate}[(a)]
\item \textbf{GPS:} GPS stands for global positioning system, which is used for infer the location of a device. GPS, embedded in IoT and CPS devices, is a passive device-- which cannot transmit anything and only capture signal from satellite. At specific time intervals, GPS satellites emit a signal containing their current position and GPS receiver of the device capture multiple signals from satellites at various times. When it receives a signal, based on the time it takes to get the packets, it can determine how far it is from the satellite. By calculating distances from various satellites, the GPS receiver can infer the correct location of the device \cite{1338639}. 
\item \textbf{Magnetic sensor:} Magnetic sensors in CPS and IoT devices have the role to fix the display position of the device in relation to Earth\textquotesingle s magnetic field. Magnetic sensor can also be used as digital compass in some devices like smartphones, navigation devices, etc.. There are usually three magnetic field sensors, perpendicular to each other, which are used to detect Earth\textquotesingle s magnetic field with respect to device peripheral. These magnetic sensors can give data for changes in the magnetic field of the surroundings of the devices.
\end{enumerate}

\begin{table*}[htb!]
\centering
\arraybackslash
\fontsize{8}{10}\selectfont
\begin{tabular}{cccc}
\toprule
\textbf{Sensor Type}    & \textbf{Sensor Name}      & \textbf{Implemented Device Name}  & \textbf{Description and Usage} \\ \hline
\midrule
\multirow{3}{*}{Motion Sensor}                                                   & Accelerometer              & \begin{tabular}[c]{@{}c@{}}Smart phone, Smart Watch, Smart Glass, \\ Home automation system, Smart TV, \\ Navigation devices, Smart cars, Smart meter\end{tabular} & \begin{tabular}[c]{@{}c@{}}An electro-mechanical device which can \\ measure changes in acceleration forces \\ along x, y, and z-axis.\\ Detect several types of motion like shake, tilt, etc. \\ and adjust the display of \\ the device accordingly.\end{tabular}    \\ \cline{2-4} 
                                                                                 & Linear Acceleration Sensor & \begin{tabular}[c]{@{}c@{}}Smart phone, Smart Watch, Smart Glass, \\ Home automation system, Smart TV, \\ Navigation devices, Smart cars, Smart meter\end{tabular} & \begin{tabular}[c]{@{}c@{}}One type of accelerometer which can detect \\ acceleration along one axis without \\ considering effect of gravitational force. \\Main purpose of using this is to \\adjust display with motion.\end{tabular}                                                                                         \\ \cline{2-4} 
                                                                                 & Gyroscope                  & \begin{tabular}[c]{@{}c@{}}Smart phone, Smart Watch, Home automation system, \\ Smart TV, Navigation devices, Smart meter\end{tabular}                             & \begin{tabular}[c]{@{}c@{}}Measures the rate of change of \\ angular momentum in all three axis. \\It detect rotational movement of the device \\ and adjust display accordingly \end{tabular}                                        \\ \hline
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Environmental \\ Sensor\end{tabular}} & Light Sensor               & \begin{tabular}[c]{@{}c@{}}Smart phone, Smart Watch, Smart Glass, \\ Home automation system, Smart TV, Smart cars\end{tabular}                                     & \begin{tabular}[c]{@{}c@{}} Usually a photodiode which change \\ characteristics with the change \\ of light intensity. Main purpose of using \\ this is to adjust brightness and \\ contrast of the display\\ of the device. Also, used to \\control automatic lighting system \end{tabular}       \\ \cline{2-4} 
                                                                                 & Proximity Sensor           & \begin{tabular}[c]{@{}c@{}}Smart phone, Smart Watch, \\ Home automation system, Navigation devices\end{tabular}                                                    & \begin{tabular}[c]{@{}c@{}}IR-based sensor to detect\\ the presence of nearby objects \\ without any physical contact. \\It is used to reduce power consumption \\of the display by turning off the\\ LCD backlight and avoid inadvertent touches. \end{tabular}\\ \cline{2-4} 
                                                                                 & Temperature Sensor         & \begin{tabular}[c]{@{}c@{}}Smart Phone, Smart Thermostat, Home automation\\ system\end{tabular}                                                                    & \begin{tabular}[c]{@{}c@{}}Measures temperature of the device \\as well as ambient temperature. \\It controls temperature in smart thermostat and \\home automation system.  \end{tabular}                                                           \\ \cline{2-4} 
                                                                                 & Audio Sensor               & \begin{tabular}[c]{@{}c@{}}Smart phone, Smart Watch, Smart Glass,\\ Home automation system, Smart TV, Smart cars,\end{tabular}       & \begin{tabular}[c]{@{}c@{}}Two types of audio sensor - microphone \\ and speaker. Microphone is used to detect \\ acoustic signal and speaker is used \\to playback audio signal. Audio sensors \\are used to detect audio signals and \\playback audio files\end{tabular}                                                                  \\ \cline{2-4} 
                                                                                 & Camera                     & \begin{tabular}[c]{@{}c@{}}Smart phone, Smart Glass, Home automation system, \\ Smart TV, Smart cars\end{tabular}                                                  & \begin{tabular}[c]{@{}c@{}}Can be considered as a combination \\ of sensors. It deals with light intensity, \\device ambiance, etc. to capture pictures\\ and videos of surroundings \\In navigation devices, camera provides \\live video feeds. \end{tabular}      \\ \hline
\multirow{2}{*}{Position Sensor}                                                 & GPS                        & \begin{tabular}[c]{@{}c@{}}Smart phone, Smart Watch,\\ Navigation devices \end{tabular}                                                                                                                     & \begin{tabular}[c]{@{}c@{}}A passive sensor which can capture \\ signal from satellite to infer the \\ location of the device. Main \\usage of GPS is in navigation systems. \end{tabular}                                                 \\ \cline{2-4} 
                                                                                 & Magnetic Sensor            & \begin{tabular}[c]{@{}c@{}}Smart phone, Smart Watch, Smart Glass, \\ Navigation devices\end{tabular}                                                               & \begin{tabular}[c]{@{}c@{}}Measures magnetic field with \\ respect to earth's magnetic field.\\ It is used as digital compass in \\ navigation devices. It is also used to \\fix display position \\ by considering magnetic field.\end{tabular}               \\
\bottomrule                                                                              
\end{tabular}
\caption{Sensors used in IoT devices}
\label{sensors}
\end{table*}

%\subsection{Power Analysis}
%Power analysis of a device refers to the power consumption rate of different parts of a device. Information related to power consumption and power flow can be easily collected by using simple tools like multimeter, oscilloscope, etc. Power analysis of a device is considered as a side channel because user does not have to exploit the normal activity of a device to acquire this information. There are different types of power analysis, such as \textit{Simple Power Analysis}, \textit{Differential Power Analysis}, \textit{High-order Differential Power Analysis}, and \textit{Correlation Power Analysis} \cite{messerges1999investigations}. Power analysis can be lead to infer the internal process going inside a device which can be useful to create an attack scenario \cite{messerges1999investigations}.

%\begin{table*}[t]
%    \centering
%\caption{Sensors in different IoT and CPS devices}
%    \begin{tabular}{| c | c | c | c | c | c | c | c | c |}

%    \hline
%    & Accelerometer & Gyroscope & Magnetometer & Light Sensor & Audio Sensor & Camera & GPS & Proximity Sensor \\ \hline
%     Smart phone & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark \\ \hline
%     Tablet & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark \\ \hline
%     Laptop & \Checkmark & \Checkmark & \Checkmark & \xmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark  \\ \hline
%	Smart Watch & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \xmark & \Checkmark & \Checkmark  \\ \hline
%	Smart Glass & \Checkmark & \xmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \xmark & \xmark  \\ \hline
%	Home Automation System & \Checkmark & \Checkmark & \xmark & \Checkmark & \Checkmark & \checkmark & \xmark & \Checkmark  \\ \hline
%	Smart TV & \Checkmark & \Checkmark & \xmark & \Checkmark & \Checkmark & \Checkmark & \xmark & \xmark  \\ \hline
%	Navigation Devices & \Checkmark & \Checkmark & \Checkmark & \xmark & \xmark & \xmark & \Checkmark & \Checkmark  \\ \hline
%	Smart Cars & \Checkmark & \xmark & \xmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \xmark  \\ \hline
%	Smart Meter & \Checkmark & \Checkmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark  \\ \hline
	

%    \end{tabular}
% \label{tab:1}
%\end{table*}
%\subsection{Electromagnetic (EM) emanation channel}
%Electromagnetic (EM) emanation is a common phenomenon for any electronic device. EM emanation occurs because of current flows within I/O, data processing unit or other parts of a device. This EM emanation depends on device\textquotesingle s electrical and physical characteristics thus varies from one device to another. Different tasks running on a device also show different but specific EM emanation. As normal activity of a device does not have to be altered to perform EM analysis, it can be considered as a side channel of a device \cite{rohatgi2009electromagnetic}.
